Low Complexity Decoding for Punctured Trellis-Coded Modulation Over Intersymbol Interference Channels

Classical trellis-coded modulation (TCM) as introduced by Ungerboeck in 1976/1983 uses a signal constellation of twice the cardinality compared to an uncoded transmission with one bit of redundancy per PAM symbol, i.e., application of codes with rates $\frac{n-1}{n}$ when $2^{n}$ denotes the cardinality of the signal constellation. The original approach therefore only comprises integer transmission rates, i.e., $R=\left\{ 2,\,3,\,4\,\ldots \right\}$, additionally, when transmitting over an intersymbol interference (ISI) channel an optimum decoding scheme would perform equalization and decoding of the channel code jointly. In this paper, we allow rate adjustment for TCM by means of puncturing the convolutional code (CC) on which a TCM scheme is based on. In this case a nontrivial mapping of the output symbols of the CC to signal points results in a time-variant trellis. We propose an efficient technique to integrate an ISI-channel into this trellis and show that the computational complexity can be significantly reduced by means of a reduced state sequence estimation (RSSE) algorithm for time-variant trellises.

==> content_md-labelingAndModulation.tex <==
Let us briefly investigate the labeling and modulation schemes.
%
For the $4$-ary natural labeling we multiply the MSB by $2$ and add the LSB,
\ie, $\ell[k]=2\text{MSB}[k]+\text{LSB}[k]$. An implementation of an ASK
modulator can be seen as unipolar binary symbols $\ell[k]$, mapped onto bipolar
symbols $a[k]$ within an alphabet of size $M$ with $a[k] =
(\ell[k]\cdot2)-(M-1)$.

Different labelings are easily incorporated, \eg, a Gray labeling can be achieved
by $\ell[k] = (1-\text{MSB}[k])(2\text{MSB}[k] + \text{LSB}[k]) + (\text{MSB}[k])
(2 \text{MSB}[k] + (1-\text{LSB}[k]))$.

Furthermore, a naturally labeled $4$-ary quadrature amplitude modulation (QAM)
can be represented using the MSB as real part and the LSB as imaginary part (or
vice versa), \eg, $a[k] = (2\text{MSB}-1) + \imag(2\text{LSB}-1)$, with
$\imag=\sqrt{-1}$. 

Alternativly, lookup tables fpr $\mathcal{L}$ and $\mathcal{M}$ can be use to
also allow more complex labelings and different modulations, \eg,
phase-shift-keying (PSK).

Becomes clear from the description, that in each state in the trellis only two
paths emerge. This allows for evaluating different labelings by means of testing
the distances of those two transitions in the trellis directly. Our findings
indicate that the average distance across all states is maximized by a Gray
labeling.


==> content_mdp.tex <==
The above description on matched coding enables the extension for
super-trellis decoding of \emph{punctured} convolutional coded transmission
over ISI-channels. Note that in the latter, the \emph{mother code} is matched
to the size of the modulation alphabet.

We first describe the encoding process and state transitions when
\emph{punctured} codes are used, and discuss the FSM for punctured
convolutional codes as well as the modifications necessary for the VA to run in
the resulting trellis. 

In addition, we will exemplarily show how to incorporate an ISI-channel into
a joint FSM.


==> content_numerical-md-std.tex <==
We first investigate the gain in computational complexity of MC when compared
to straightforward STD. Recall, that MC implements MLSE and therefore performs
equally to STD. The gain in computational complexity depends on the size of the
modulation alphabet and the length of the ISI-channel~(\cf, \ref{eq:complMC}).
Further reduction can be achieved via RSSE resulting in some looses in minimum
Euclidean distance.

\begin{figure}
 \begin{center}
  \begin{tikzpicture}
   \begin{axis}[
                width=.49\textwidth,
                height=7cm,
                xlabel={$10\log_{10}\left(\frac{E_b}{N_0}\right)$ in dB},
                ylabel={Complexity},
                %enlargelimits=true,
                ymode=log,
                log basis y=2,
                %ytick={2,4,8,16,32,64,128,256,512},
                %cycle list name=colors,
                cycle list={
                            every mark/.append style={fill=black},mark=*\\%
                            every mark/.append style={fill=black},mark=star\\%
                            every mark/.append style={fill=black},mark=square\\%
                           },
                grid=both,
                xmin=6,xmax=20,
                ymin=0,ymax=4048,
               ]
    \addplot table[x index=0,y index=1] {data/JOURNAL-Complexity-Comparison-complexity-1-1.csv};
    \draw[densely dashed,fill] (axis cs:6.6066066e+00,128) -- (axis cs:6.6066066e+00,2048) node {$\times$};
    % \addplot table[x index=0,y index=1] {data/JOURNAL-Complexity-Comparison-complexity-1-2.csv};
    \addplot coordinates {(1.2712713e+01,4.8000000e+01)}
       node[pos=0,pin=-30:{\footnotesize{DFSE(hard)+VA}}] {};
    % \addplot table[x index=0,y index=1] {data/JOURNAL-Complexity-Comparison-complexity-1-3.csv};
    \addplot coordinates {(9.1591592e+00,1.4400000e+02)}
       node[pos=0,pin=30:{\footnotesize{BCJR (soft)+VA}}] {};
    %\addlegendentry{MD/RSSE}
    %\addlegendentry{Hard eq + De}
    %\addlegendentry{Soft eq + De}
    \node[draw,fill=white,anchor=south east,font={\footnotesize}] at (rel axis cs:0.95,0.05) {$\mathrm{BER} = 10^{-3}$};
     \draw[thick,densely dashed,black] (axis cs:5,2048) --
                                             node[anchor=south east,pos=1]
                                             {\footnotesize{nr. of MLSE states in super-trellis}}
                                             (axis cs:14,2048);
     \draw[thick,densely dashed,black] (axis cs:5,128) --
                                             node[anchor=south east,pos=1]
                                             {\footnotesize{nr. of MLSE states in MD}}
                                             (axis cs:19,128);
   \end{axis}
  \end{tikzpicture}
 \end{center}
 \caption{Computational complexity (logarithmic scale) of an ASK modulated
          transmission ($R_\mathrm{c}=\frac12$, $\nu=4$, $g=[21,\,37]$, Gray
          labeling) over a memory-$2$ AWGN-ISI channel with linearly decreasing
          coefficients.}
 \label{fig:complexityComparison}
\end{figure}

Fig.~\ref{fig:complexityComparison} illustrates the required signal-to-noise
ratio for a bit error rate of $\mathrm{BER}=10^{-3}$ against the computational
complexity. It becomes clear that our approach achieves MLSE performance with
much fewer states then cross-product super trellis. The results also indicate
that RSSE is an efficient technique to reduce the computational complexity
without major loss in BER performance.

